EmoSet: A Large-scale Visual Emotion Dataset with Rich Attributes

Visual Emotion Analysis (VEA) aims at predicting people's emotional responses to visual stimuli. This is a promising, yet challenging, task in affective computing, which has drawn increasing attention in recent years. Most of the existing work in this area focuses on feature design, while little attention has been paid to dataset construction. In this work, we introduce EmoSet, the first large-scale visual emotion dataset annotated with rich attributes, which is superior to existing datasets in four aspects: scale, annotation richness, diversity, and data balance. EmoSet comprises 3.3 million images in total, with 118,102 of these images carefully labeled by human annotators, making it five times larger than the largest existing dataset. EmoSet includes images from social networks, as well as artistic images, and it is well balanced between different emotion categories. Motivated by psychological studies, in addition to emotion category, each image is also annotated with a set of describable emotion attributes: brightness, colorfulness, scene type, object class, facial expression, and human action, which can help understand visual emotions in a precise and interpretable way. The relevance of these emotion attributes is validated by analyzing the correlations between them and visual emotion, as well as by designing an attribute module to help visual emotion recognition. We believe EmoSet will bring some key insights and encourage further research in visual emotion analysis and understanding. Project page: https://vcc.tech/EmoSet.

==> src/07-figure.tex <==



\begin{figure*}
	\centering
	\includegraphics[width=0.888\linewidth]{figs/attr.jpg}
	%	\includegraphics[width=0.95\linewidth]{figs/annotation_tool.png}
		\vspace{-5pt}
	\caption{Visualization of emotion attributes. Each color represents one of the six attributes. Within each attribute, images and texts below show the top-k attribute values, where numbers in brackets indicate the correlation between specific values and corresponding emotions.}
	%	\Description{}
	\label{fig:att_vis}
	%	\vspace{-10pt}
\end{figure*}




==> src/stat.tex <==
\begin{table*}
	\centering
	%	\normalsize
	\footnotesize
	\caption{Statistics of eight emotion categories compared with other VEA datasets.}
	\label{tab:emo_dist}
	\renewcommand\arraystretch{1.08}
	\begin{tabular}{lccccccccl}
		\toprule
		Dataset & Amusement & Anger & Awe & Contentment & Disgust & Excitement & Fear & Sadness & Total\\
		\midrule
		IAPSa & 37 (9\%) & \textcolor{blue}{8 (2\%)} & 54 (14\%) & 63 (16\%) & \textcolor{red}{74 (19\%)} & 55 (14\%) & 42 (11\%) & 62 (16\%) & 395 \\
		Artphoto & 101 (13\%) & 77 (10\%) & 102 (13\%) & 70 (9\%) & \textcolor{blue}{70 (9\%)} & 105 (13\%) & 115 (14\%) & \textcolor{red}{166 (21\%)} & 806 \\
		Abstract & 25 (11\%) & \textcolor{blue}{3 (1\%)} & 15 (7\%) & \textcolor{red}{63 (28\%)} & 18 (8\%) & 36 (16\%) & 36 (16\%) & 32 (14\%) & 228 \\
		FI & 4942 (21\%) & 1266 (5\%) & 3151 (14\%) & \textcolor{red}{5374 (23\%)} & 1658 (7\%) & 2963 (13\%) & \textcolor{blue}{1032 (4\%)} & 2922 (13\%) & 23308 \\
		\textbf{EmoSet} & 19445 (16\%) & \textbf{\textcolor{blue}{10660 (9\%)}} & 15037 (13\%) & 16337 (14\%) & 10666 (9\%) & \textbf{\textcolor{red}{19828 (17\%)}} & 13453 (11\%) & 12676 (11\%) & \textbf{118102} \\
		\bottomrule
	\end{tabular}
	\vspace{-10pt}
 \label{tab:stat}
\end{table*}

==> table/att.tex <==
\begin{table*}[h!]   % 表格中不带引用
	\setlength{\abovecaptionskip}{0.1cm} 
	\setlength{\belowcaptionskip}{0.1cm}
	\tabcolsep=1cm
	\scriptsize
	%	\scriptsize
	%	\tiny
	\renewcommand\arraystretch{1.2}  % 行间距
	\setlength\tabcolsep{2.5pt}   % 列间距
	\centering
	\caption{Top-3 attributes for different emotions.}
	\label{tab:att}
	\begin{tabular}{cllll}
		\toprule
		Emotion & Scene & Object & Human action \\
		\midrule
		Amusement & Carousel, Amusement park, Delicatessen & Christmas tree, Doll, Tomato & Decorating the Christmas tree, Belly dancing, Dining \\
		Awe & Mountain snowy, Valley, Waterfall &  Castle, Airplane, Eagle  & Answering questions, Driving car, Skiing \\
		Contentment & Lawn, Beach, Park & Goose, Coffee, Duck & Baby waking up, Petting cat, Reading book \\
		Excitement & Stage, Wave, Football field & Surfboard, Guitar, Paddle  & Water skiing, Playing ice hockey, Side kick \\
		Anger  & Boxing ring, Plaza, Forest & Lion, Leopard, Tiger & Extinguishing fire, Finger snapping, Pumping fist \\
		Disgust & Landfill, Underwater, Butchers shop & Caterpillar, Waste container, Snake & Garbage collecting, Smoking, Unloading truck \\
		Fear & Corridor, Staircase, Forest & Skull, Lantern, Stairs & Holding snake, Scuba diving, Texting \\
		Sadness & Cemetery, Mausoleum, Stable & Bust, Bronze sculpture, Handbag & Massaging persons head, Smoking, Digging \\
		\bottomrule
	\end{tabular}
\end{table*}

==> table/attr_top3.tex <==
\begin{table*}[h!]   % 表格中不带引用
\setlength{\abovecaptionskip}{0.1cm} 
\setlength{\belowcaptionskip}{0.1cm}
\tabcolsep=1cm
% \footnotesize
\scriptsize
% \tiny
\renewcommand\arraystretch{1.2}  % 行间距
\setlength\tabcolsep{1.5pt}   % 列间距
\centering
\caption{Top-3 attribute values in scene type, object class and human action.}
\begin{tabular}{llll}
    \toprule[1pt]
    Emotion &  Scene type  & Object class & Human action  \\
    \midrule[0.5pt]
    Amusement &   Carousel, Amusement park, Delicatessen &Christmas tree, Doll, Tomato   & Decorating the christmas tree, Belly dancing, Dining \\
    Awe        & Mountain snowy, Valley, Waterfall      &  Castle, Airplane, Eagle  & Answering questions, Driving car, Skiing \\
    Contentment  & Lawn, Beach, Park    & Goose, Coffee, Duck  & Baby waking up, Petting cat, Reading book \\
    Excitement  & Stage, Wave, Football field    & Surfboard, Guitar, Paddle  & Water skiing, Playing ice hockey, Side kick \\
    Anger      & Boxing ring, Plaza, Forest   & Lion, Leopard, Tiger & Extinguishing fire, Finger snapping, Pumping fist \\
    Disgust     & Landfill, Underwater, Butchers shop      & Caterpillar, Waste container, Snake  & Garbage collecting, Smoking, Unloading truck \\
    Fear      & Corridor, Staircase, Forest & Skull, Lantern, Stairs  & Holding snake, Scuba diving, Texting \\
    Sadness   & Cemetery, Mausoleum, Ruin   & Bust, Bronze sculpture, Handbag & Massaging persons head, Smoking, Digging  \\
    \bottomrule[1pt]
\end{tabular}
\end{table*}


